A Systematic Evaluation of Generated Time Series and Their Effects in Self-Supervised Pretraining

Self-supervised Pretrained Models (PTMs) have demonstrated remarkable performance in computer vision and natural language processing tasks. These successes have prompted researchers to design PTMs for time series data. In our experiments, most self-supervised time series PTMs were surpassed by simple supervised models. We hypothesize this undesired phenomenon may be caused by data scarcity. In response, we test six time series generation methods, use the generated data in pretraining in lieu of the real data, and examine the effects on classification performance. Our results indicate that replacing a real-data pretraining set with a greater volume of only generated samples produces noticeable improvement.

==> insert/tab_summary_uea.tex <==
% \begin{table*}[!ht]
%     \centering
%     \caption{The results are the average rank for each configuration of experiments, one of the backbone models, one of the PTMs, and one of the data generators during pretraining. There are 30 datasets in the UEA Archive[CITE].}
%     \begin{tabular}{l|c||c|ccc|ccc}
%     \hline
%         \textbf{Backbone} & \textbf{PTM} & \textbf{NG} & \textbf{RW} & \textbf{SW} & \textbf{MG} & \textbf{GAN} & \textbf{$\beta$-VAE} & \textbf{Diff.} \\ \hline \hline
%         1NN ED & N/A & 34.85 & - & - & - & - & - & - \\ 
%         1NN DTW & N/A & 29.50 & - & - & - & - & - & - \\ \hline
%         \multirow{4}{*}{ResNet} & N/A & 25.17 & - & - & - & - & - & - \\
%         ~ & MixingUp & 20.48 & 23.98 & 22.22 & \textbf{18.47} & 20.57 & 22.70 & \underline{20.38} \\ 
%         ~ & TimeCLR & 22.80 & \underline{21.33} & 21.35 & 23.28 & \textbf{20.95} & 23.78 & 25.45 \\
%         ~ & TS2Vec & 22.18 & 22.22 & 22.02 & 23.78 & 26.73 & \underline{21.27} & \textbf{20.78} \\ \hline
%         \multirow{4}{*}{Transformer} & N/A & 23.10 & - & - & - & - & - & - \\
%         ~ & MixingUp & 25.70 & 23.07 & 24.77 & \underline{22.72} & 22.92 & 22.87 & \textbf{22.48} \\
%         ~ & TimeCLR & 25.23 & \textbf{22.03} & \underline{23.43} & 25.12 & 23.90 & 24.73 & 23.62 \\
%         ~ & TS2Vec & 23.70 & \underline{23.68} & 25.17 & 24.85 & 24.22 & 25.75 & \textbf{21.70} \\ 
%     \end{tabular}
%     \label{tab:summary_uea}
% \end{table*}

\begin{table*}[!t]
    \centering
    \caption{The results are the average rank for each configuration of experiments, one of the backbone models, one of the PTMs, and one of the data generators during pretraining. 
    There are 30 datasets in the UEA Archive~\cite{bagnall2018uea}.}
    \footnotesize
    \begin{tabular}{l|l||c|ccc|ccc}
    \hline
        \textbf{Backbone} & \textbf{PTM} & \textbf{NG} & \textbf{RW} & \textbf{SW} & \textbf{MG} & \textbf{GAN} & \textbf{$\beta$-VAE} & \textbf{Diff.} \\ \hline \hline
        1NN ED & N/A & 43.87 & - & - & - & - & - & - \\ 
        1NN DTW & N/A & 36.42 & - & - & - & - & - & - \\ \hline
        \multirow{5}{*}{ResNet} & N/A & 30.13 & - & - & - & - & - & - \\
        ~ & TimeCLR & 27.38 & 25.60 & \underline{25.57} & 28.15 & \textbf{25.08} & 28.73 & 30.87 \\ 
        ~ & TS2Vec & 26.75 & 26.73 & 26.00 & 28.82 & 32.32 & \underline{25.42} & \textbf{25.27} \\
        ~ & MixingUp & 24.92 & 29.25 & 27.07 & \textbf{22.53} & \underline{24.53} & 27.53 & 24.75 \\ 
        ~ & TF-C & \textbf{38.92} & 41.43 & 45.12 & 43.10 & \underline{41.02} & 44.93 & 41.57 \\ \hline
        \multirow{5}{*}{Transformer} & N/A & 26.92 & - & - & - & - & - & - \\ 
        ~ & TimeCLR & 29.43 & \textbf{26.22} & \underline{27.58} & 29.68 & 28.30 & 28.72 & 27.67 \\ 
        ~ & TS2Vec & \underline{27.57} & 27.63 & 29.58 & 29.43 & 28.30 & 29.97 & \textbf{25.43} \\ 
        ~ & MixingUp & 30.35 & 26.95 & 29.12 & 26.90 & \underline{26.72} & 26.98 & \textbf{26.03} \\ 
        ~ & TF-C & 33.88 & 34.13 & \underline{32.75} & 38.25 & \textbf{32.52} & 34.67 & 38.55 \\  \hline
    \end{tabular}
    \label{tab:summary_uea}
\end{table*}
